Lagrangian Particle Classification and Lagrangian Flux Identities for a Moving Hypersurface

For a moving hypersurface in the flow of a nonautonomous ordinary differential equation in $n$-dimensional Euclidean spaces, the fluxing index of a passively-advected Lagrangian particle is the total number of times it crosses the moving hypersurface within a time interval. The problem of Lagrangian particle classification is to decompose the phase space into flux sets, equivalence classes of Lagrangian particles at the initial time. In the context of scalar conservation laws, the problem of Lagrangian flux calculation (LFC) is to find flux identities that relate the Eulerian flux of a scalar through the moving hypersurface, a spatiotemporal integral over the moving surface in a given time interval, to spatial integrals over donating regions at the initial time of the interval. In this work, we implicitly characterize flux sets via topological degrees, explicitly construct donating regions, prove the equivalence of flux sets and donating regions, and establish two flux identities; these analytical results constitute our solutions to the aforementioned problems. Based on a flux identity suitable for numerical calculation, we further proposed a new LFC algorithm, proved its convergence, and demonstrated its efficiency, good conditioning, and high-order accuracy by results of various numerical tests.

==> sec/obsolete.tex <==
\section{From winding numbers to topological degrees}
\label{sec:from-winding-number}

\subsection{Winding numbers}
\label{sec:winding-numbers}

A \emph{closed curve} %$\Gamma\subset\mathbb{R}^2$
 is the image of a continuous function
 $\gamma: [0, 2\pi]\rightarrow \mathbb{R}^2$
 with $\gamma(0)=\gamma(2\pi)$.
A \emph{Jordan curve} is a closed curve $\Gamma$
 whose parametrized function $\gamma$
 is injective on $[0,2\pi)$.
The Jordan curve theorem states that
 $\mathbb{R}^2\setminus \Gamma$ consists of
 only two components, one bounded and one unbounded,
 with $\Gamma$ being their common boundary.
A Jordan curve $\Gamma$ is \emph{positively oriented}
 if $\BCJ(\Gamma)$, the bounded complement of $\Gamma$,
 always lies to the left of an observer who traverses $\Gamma$
 according to $\gamma$;
 otherwise it is \emph{negatively oriented}. 

A closed curve can be viewed as the image
 of a Jordan curve $\Gamma$ under a continuous map
 $f: \mathbb{R}^2\rightarrow\mathbb{R}^2$.
The \emph{winding number of an oriented closed curve} $f(\Gamma)$
 around a point $a\in \mathbb{C}\setminus f(\Gamma)$
 is the number of times it encircles $a$,
 i.e., 
 \begin{equation}
   \label{eq:windingNumber}
   w(f(\Gamma),a) := \frac{1}{2\pi\ii}
   \int_{f(\Gamma)} \frac{\dif z}{z-a}, 
 \end{equation}
 where $\ii=\sqrt{-1}$.
It can be shown \cite[p. 203]{rudin86:_real_compl_analy}
 that $w(f(\Gamma),z)$ %$\in\mathbb{Z}$ %must be an integer
 is a constant integer in each connected component of
 $\mathbb{C}\setminus f(\Gamma)$.
In particular, we have 
  \begin{equation}
    \label{eq:windingNumberJordan}
    w(\Gamma,a) =
    \begin{cases}
      +1 & \text{if $a\in \BCJ(\Gamma)$
        and $\Gamma$ is positively oriented},
      \\
      -1 & \text{if $a\in \BCJ(\Gamma)$ and $\Gamma$ is negatively oriented},
      \\
      0  & \text{if $a$ belongs to the unbounded complement of $\Gamma$}.
    \end{cases}
  \end{equation}

A \emph{free homotopy}  in $\mathbb{R}^2$ between two closed curves
  parametrized as $\gamma_1$ and $\gamma_2$ % in $\mathbb{R}^2$
  is a function $H_f:[0,1]\times[0,2\pi]\rightarrow \mathbb{R}^2$
  such that $H_f(0,\theta)=\gamma_1(\theta)$
  and $H_f(1,\theta)=\gamma_2(\theta)$
  for all $\theta$,
  and $H_f(t,0)=H_f(t,2\pi)$ for all $t$.
 Then $\gamma_1$ and $\gamma_2$ 
 are said to be \emph{freely homotopic}
 in $\mathbb{R}^2$. %$ \setminus \mathbf{x}$.

\begin{theorem}[Hopf \cite{hopf35:_ueber_drehun_tangen_sehnen_kurven}]
  \label{thm:Hopf}
  Let a point $a\in \mathbb{R}^2$ be given.
  Two closed curves $\gamma_1$ and $\gamma_2$
  are freely homotopic in $\mathbb{R}^2\setminus\{a\}$
  if and only if
  $w(\gamma_1, a) = w(\gamma_2, a)$.
\end{theorem}

The Hopf theorem is the most essential characterization
of winding numbers. 

\subsection{The argument principle}
\label{sec:argument-principle}

We denote by $\overline{S}$ the closure of a point set $S$.

\begin{theorem}[Argument principle]
  \label{thm:argumentPrincipleAnalytic}
  For an oriented Jordan curve $\Gamma$,
  an analytic map 
  $f:\overline{\textrm{BCJ}(\Gamma)}\rightarrow\mathbb{C}$, 
  and a point $a\not\in f(\Gamma)$, 
  we have 
  \begin{equation}
    \label{eq:argumentPrincipleAnalytic}
    w(f(\Gamma),a) = \sum_{z_j\in f^{-1}(a)} w(\Gamma,z_j) m_j,
  \end{equation}
  where $m_j$ is the algebraic multiplicity of the preimage $z_j$. 
%  and $\overline{\cdot}$ denotes the closure of a point set.
\end{theorem}

% Since an analytic function is locally equivalent
%  to its power series,
%  the multiplicity $m_j$ in (\ref{eq:argumentPrincipleAnalytic})
%  is the algebraic multiplicity of $f$. 

Theorem \ref{thm:argumentPrincipleAnalytic} furnishes an explicit
 algorithm for locating solutions of the equation
 $f(x)=a$: % preimage of $a$ under an \emph{analytic} map $f$: 
 draw a positively oriented Jordan curve $\Gamma$,
 map $\Gamma$ to the closed curve $f(\Gamma)$,
 and deduce from (\ref{eq:windingNumberJordan}) and 
 (\ref{eq:argumentPrincipleAnalytic}) that
 $w(f(\Gamma),a)$ equals the number of preimages of $a$
 in BCJ$(\Gamma)$, 
 counted with their algebraic multiplicity.

The algebraic multiplicity of a root $z_j$ of $a$
 is an essential characterization
 of the local behavior of $f$ at $z_j$.
But what if $f$ is not analytic but merely continuous?
In this case, 
the concept of algebraic multiplicity
does not even apply. % to continuous functions.

Let $\Gamma_j$ be a positively oriented Jordan curve
 such that BCJ$(\Gamma_j)$
 contains $z_j$ and no other preimages of $a=f(z_j)$.
For another Jordan curve $\tilde{\Gamma}_j$ satisfying the same
 conditions, 
 Hopf's theorem implies $w(f(\tilde{\Gamma}_j), a)=w(f(\Gamma_j), a)$. 
Hence we have an equivalence class of
 oriented Jordan curves
 whose images characterize the local behavior of $f$ at $z_j$
 as a topological invariant, 
 which is called the \emph{topological multiplicity}
 of a continuous function $f$:  %$\in{\mathcal C}(\mathbb{C})$ at $z_j$,
 \begin{equation}
    \label{eq:topoMultiplicityDef}
    \nu_f(z_j) := w(f(\Gamma_j), f(z_j)). 
 \end{equation}
 % where $\Gamma_j$ is a positively oriented Jordan curve
 % such that BCJ$(\Gamma_j)$
 % contains $z_j$ and no other preimages of $a=f(z_j)$.
It follows from  Hopf's theorem that, 
 for $f:\overline{\textrm{BCJ}(\Gamma)}\rightarrow\mathbb{C}$
 and a point $a\not\in f(\Gamma)$,
 \begin{equation}
   \label{eq:argumentPrincipleCont}
   w(f(\Gamma),a) = \sum_{z_j\in f^{-1}(a)} w(\Gamma,z_j) \nu_f(z_j),
 \end{equation}
 where $\Gamma$ is positively oriented
 and $\nu_f(z_j)$ is the topological multiplicity
 of $f$ in (\ref{eq:topoMultiplicityDef}).


\subsection{What is so special about analytic maps?}
\label{sec:specialtyOfAnalyticMaps}

Given the striking similarity
 between (\ref{eq:argumentPrincipleCont})
 and (\ref{eq:argumentPrincipleAnalytic}), 
 it is natural to ask: %So in the set of continuous functions
 what distinguishes analytic maps from continuous maps? 
% $f: \mathbb{C}\rightarrow \mathbb{C}$?

First,
the algorithm of determining the number of solutions of $f(x)=a$
(see the paragraph
after Theorem \ref{thm:argumentPrincipleAnalytic})
does not work any more.
For a continuous map $f$,
the strongest statement of such nature is
\begin{equation}
  \label{eq:numberOfSolutionsCont}
  w(f(\Gamma),a)\ne 0 \ \Rightarrow\
  f^{-1}(a)\cap \textrm{BCJ}(\Gamma)\ne \emptyset.
\end{equation}

This weakening of (\ref{eq:argumentPrincipleAnalytic})
 and (\ref{eq:windingNumberJordan}) to (\ref{eq:numberOfSolutionsCont})
 is due to the fact that,
 in contrast to the algebraic multiplicity of an analytic map
 being always nonnegative,
 the topological multiplicity of a continuous map
 can be both positive and negative.
For example, the complex map $f(x+\ii y)=x+\ii |y|$
 with $x,y\in \mathbb{R}$
 is not analytic but continuous,
 and the equation $f(z) = a\ii$ with $a>0$
 has two solutions $z=\pm a\ii$. 
For a positively oriented
 Jordan curve $\Gamma$ with $\pm a\ii\in \text{BCJ}(\Gamma)$, 
 we have $w(f(\Gamma),a\ii)= 0$, 
 yet $\nu_f(a\ii)=+1\ne 0$ and $\nu_f(-a\ii)=-1\ne 0$. 

Second, in $\mathbb{R}^2$ analytic maps preserve orientations
 while continuous functions do not.
For example, the complex conjugate $z\mapsto \overline{z}$
 flips the orientation of every oriented Jordan curve in $\mathbb{C}$.

 \begin{lemma}
   \label{lem:orientationPreserved}
%   For $z_0\in\mathbb{C}$,
   An analytic function $f:\mathbb{C}\rightarrow\mathbb{C}$
   with $J_f(z_0)\ne 0$
   has $J_f(z_0)>0$. 
%   preserves the orientation of sufficiently small
   In other words, it maps an infinitesimal circle
   $\varphi(\theta)=z_0 + r e^{\ii \theta}$
   to another infinitesimal circle $\psi(\theta) = a + R e^{\ii\theta}$
   so that the Jordan curves $\varphi([0,2\pi])$ and $\psi([0,2\pi])$ 
   have the same orientation.
 \end{lemma}
 \begin{proof}
   Since $f$ is analytic and $J_f\ne 0$, $R$ is a positive constant.
   Then we have 
   \begin{displaymath}
    \psi(\theta) - a = f(\varphi(\theta)) - f(z_0)
    = f'(z_0) [\varphi(\theta) - z_0] + O(r^2), 
  \end{displaymath}
  the derivative of which yields
  $[\psi(\theta) - a]'
  = f'(z_0) [\varphi(\theta) - z_0]' + O(r)$.
  Since the cross product of two planar vectors
  $\mathbf{u},\mathbf{v}$ %in $\mathbb{R}^3$
  is given by
  $    \mathbf{u}\times\mathbf{v}
    := (0, 0, \det [\mathbf{u}, \mathbf{v}])^T$,
  % \begin{displaymath}
  %   \forall \mathbf{u},\mathbf{v}\in\mathbb{R}^2,
  %   \quad
  %   \mathbf{u}\times\mathbf{v}
  %   := (0, 0, \det [\mathbf{u}, \mathbf{v}])^T\in\mathbb{R}^3, 
  % \end{displaymath}
  we have $(A\mathbf{u})\times(A\mathbf{v})
  = (0,0,\det A \det[\mathbf{u}, \mathbf{v}])^T$
  for any matrix $A\in \mathbb{R}^{2\times 2}$.
  Therefore, the orientation of the circle $\psi$
  is related to that of $\varphi$ by 
  \begin{displaymath}
    [\psi(\theta) - a]\times [\psi(\theta) - a]'
    = (J_f(z_0)+O(r^2))[\varphi(\theta) - z_0]\times [\varphi(\theta) - z_0]',
  \end{displaymath}
  where $J_f(z_0)=\det f'(z_0)$. 
  By the Cauchy-Riemann equation, we have
  \begin{displaymath}
    f'(z_0) = 
    \begin{bmatrix}
      \alpha & -\beta \\  \beta & \alpha
    \end{bmatrix}
    \quad \Rightarrow\quad
    J_f(z_0)=\det f'(z_0) = \alpha^2+\beta^2 > 0. \qedhere
  \end{displaymath}
 \end{proof}

Lastly, the winding number of the image of a Jordan curve
 under an analytic map $f$
 may be expressed in terms of the Jacobian determinants of $f$.
 
Recall that a point $x_0\in \Omega\subset \mathbb{R}^n$ is a \emph{critical point}
  of a continuously differentiable map 
  $f:\Omega\rightarrow \mathbb{R}^n$
  if $\det f'(x_0)=0$.
A point $a\in\mathbb{R}^n$ is called a \emph{regular value}
  of $f$ %$f:\Omega\rightarrow \mathbb{R}^n$
  if $f^{-1}(a)$ contains no critical points of $f$; 
  otherwise it is a \emph{singular value} of $f$. 

\begin{corollary}
  \label{coro:windingNumberInTermsOfJf}
  For an oriented Jordan curve $\Gamma$, 
  an analytic map
  $f: \overline{\textrm{BCJ}(\Gamma)}\rightarrow\mathbb{C}$,
  and a regular value $a$ of $f$ satisfying $a\not\in f(\Gamma)$, 
  we have
  \begin{equation}
    \label{eq:windingNumberViaJacobian}
    w(f(\Gamma),a) = \sum_{z_j\in f^{-1}(a)} \sgn J_f(z_j).
  \end{equation}
\end{corollary}
\begin{proof}
  When $\Gamma$ is oriented positively or negatively,
  Lemma \ref{lem:orientationPreserved} and $J_f(z_j)\ne 0$
%  $a$ being a regular value of $f$
  imply that $\sgn J_f(z_j)=+1$ or $-1$, 
  respectively.
  Each $z_j$ has its algebraic multiplicity $m_j=1$.
  The rest follows from Theorem \ref{thm:argumentPrincipleAnalytic}
  and (\ref{eq:windingNumberJordan}). 
\end{proof}


\subsection{Sphere eversion in $\mathbb{R}^3$
and a crucial difference of LFC in 2D and 3D}
\label{sec:sphere-eversion}

An analytic map
$f: \mathbb{R}^2\rightarrow \mathbb{R}^2$
 preserves orientation and 
 simplifies the matter of orienting a Jordan curve: 
 the outward normal vector can be determined
 \emph{once and for all} as pointing from the bounded complement
 to the unbounded complement.
Since a diffeomorphic flow map
 never turns the Jordan curve inside out, 
 this \emph{extrinsic} choice of the normal direction 
 always comply with the convention of LFC that
 flux be calculated from one side to the other.
In addition, 
 this extrinsic orientation simplifies LFC for a Jordan curve: 
 then the only nonzero donating regions are 
 $\mathcal{D}_{\mathcal{S}}^{+1} (t_{0},k)$
 and $\mathcal{D}_{\mathcal{S}}^{-1} (t_{0},k)$. 
 Indeed, to cross the Jordan curve from one complement
 to the other twice, 
 a particle must return to its original complement, 
 but then this extrinsic orientation
 implies that the fluxing index be zeroed out 
 before the second crossing. 
 Consequently, 
 the Lagrangian flux reduces to
\cite[Corollary 10]{zhang2013highly}
\begin{displaymath}
%  \label{eq:flux2DforJordan}
  \int_{t_0}^{t_0+k} \int_{\mathcal{S} (t)}
  f(\mathbf{x},t) \bigl[
  \mathbf{u} (\mathbf{x},t) -\partial_{t}\mathcal{S}
  \bigr] \cdot \mathbf{n} (\mathbf{x},t) \dif \mathbf{x} \dif t
  =  \int_{\mathcal{D}_{\mathcal{S}}^{1} (t_{0},k)}
  f (\mathbf{x},t_{0})\,\dif \mathbf{x}
  -  \int_{\mathcal{D}_{\mathcal{S}}^{-1} (t_{0},k)}
  f (\mathbf{x},t_{0})\, \dif \mathbf{x}.
\end{displaymath}
In particular, provided that
two moving Jordan curves coincide both at $t_0$ and at $t_e$, 
their Lagrangian fluxes are the same.

This orientation-preserving property of an analytic map
 $f: \mathbb{C}\rightarrow \mathbb{C}$
 depends on the fact of the dimensionality
 of $\mathbb{C}\simeq \mathbb{R}^2$ being 2,
 c.f. Lemma \ref{lem:orientationPreserved}. 
In dramatic contrast, an analytic map
 $f:\mathbb{R}^3 \rightarrow \mathbb{R}^3$
 need not preserve the orientation of 
 a simple closed surface.

A celebrated example is sphere eversion,
 the process of turning a sphere inside out in $\mathbb{R}^3$.
Counter-intuitively, a diffeomorphic flow map
 may turn a sphere inside out 
 (with potential self-intersections)
 without tearing or creasing on the sphere.
% However, the two-dimensional analogy that turning a circle
% inside out smoothly and continuously is not possible.
% These surprising results can be viewed as a veridical paradox,
% which is true but appears to be false at first glance.
The first existence proof of sphere eversion
is due to Smale \cite{smale1959classification}
and the first constructed example was exhibited by
Shapiro and Morin \cite{francis1980arnold}.
There is an excellent video of
 sphere eversion created by Levy and Thurston \cite{levy1995making}
 using the ``belt-trick.''
For recent developments of sphere eversion, 
 the reader is referred to \cite{litman2017sphere}. 

What is the consequence of sphere eversion on LFC in $\mathbb{R}^3$?  
Clearly 
 it is no longer appropriate 
 to choose the normal direction of a simple closed surface
 to point from the bounded complement to the unbounded complement, 
 i.e., 
 extrinsically orienting a hypersurface via features
 of the embeding space does not work any more.
 
As a simple counterexample,
 we assume $\mathbf{u} (\mathbf{x},t) =\mathbf{0}$
 and $f (\mathbf{x},t) =1$.
Then the flow map is the identity 
$\phi_{t_{0}}^{t}(\mathbf{x})=\mathbf{x}$.
Consider two simple closed surfaces.
The first is the unit sphere fixed for all $t\in [t_{0},t_{0}+k]$;  
the corresponding flux is clearly zero.
The second is a sphere turned inside out once in $[t_{0},t_{0}+k]$
but coincide with the unit sphere both at $t_0$ and $t_0+k$;
in this case we have
\begin{displaymath}
  \int_{t_0}^{t_0+k} \int_{\mathcal{S}_{2} (t)}
  f(\mathbf{x},t) \bigl[
  \mathbf{u} (\mathbf{x},t) -\partial_{t}\mathcal{S}_{2}
  \bigr] \cdot \mathbf{n} (\mathbf{x},t)\, \dif \mathbf{x} \dif t
  =2 \int_{\mathcal{D}_{\mathcal{S}_{2}}^{2} (t_{0},k)}
  f (\mathbf{x},t_{0})\dif \mathbf{x}
  = \frac{8}{3}\pi,
\end{displaymath}
where 
$\mathcal{D}_{\mathcal{S}_{2}}^{2} (t_{0},t_{e})=\left\{ \mathbf{x}|
  |\mathbf{x}|  < 1 \right\}$ is the unit ball. 

To sum up,
 the generalization of LFC from 2D to 3D is not straightforward, 
 because it is no longer adequate
 to adopt the extrinsic choice of the normal direction
 for a simple closed hypersurface.
To account for the potential dependence of normal vector
 upon the velocity field,
 we must have a coordinate system
 in which the moving surface is oriented \emph{intrinsically}.

 
\subsection{The topological degree}
\label{sec:topological-degree}

%The topological degree is a
The generalization
 of the winding number to $\mathbb{R}^n$
 starts from axiomizing its three key features, 
 which leads to 
 
\begin{theorem}
  \label{thm:topoDegreeRnExistence}
  There is at most one function $\deg: M\rightarrow\mathbb{Z}$, where 
  \begin{equation}
    \label{eq:topoDegreeRn}
    M:= \left\{(f,\Omega,y):
      \left\{
    \begin{array}{l}
      \Omega\subset \mathbb{R}^n \text{ open and bounded};
      \\
      f: \overline{\Omega} \rightarrow \mathbb{R}^n \text{ continuous};
      \\
      y\in \mathbb{R}^n \setminus f(\partial\Omega)
    \end{array}\right.
    \right\}, 
  \end{equation}
  that satisfies normalization, additivity, and homotopy, i.e., 
  \begin{enumerate}[(TPD-1)]\itemsep0em
  \item $\deg(I,\Omega, y)=1$ for all $y\in\Omega$
    where $I$ is the identity map; 
  \item $\deg(f,\Omega,y) = \deg(f,\Omega_1,y) + \deg(f,\Omega_2,y)$
    whenever $\Omega_1$ and $\Omega_2$
    are disjoint open subsets of $\Omega$ such that
    $y\not\in f(\overline{\Omega}\setminus(\Omega_1\cup\Omega_2))$;
  \item $\deg(H(t,\cdot), \Omega, y(t))$
    is independent of $t\in[0,1]$ whenever 
    $H:[0,1]\times\overline{\Omega}\rightarrow \mathbb{R}^n$
    is continuous, 
    $y:[0,1]\rightarrow \mathbb{R}^n$ is continuous,
    and $y(t)\not\in H(t,\partial\Omega)$
    for all $t\in[0,1]$. 
  \end{enumerate}
\end{theorem}
\begin{proof}
  See \cite[\S 1]{deimling10:_nonlin_funct_analy}.
\end{proof}

% In (\ref{eq:topoDegreeRn}),
%  the $n$-dimensional domain $\Omega$ corresponds
%  to two-dimensional BCJ$(\Gamma)$ of a Jordan curve $\Gamma$. 

Such a function is constructed as follows.

\begin{definition}[Topological degree]
  \label{def:topoDegree}
  First, the \emph{topological degree} of $(f,\Omega, y_1)\in M$
  with $f\in {\mathcal C}^1(\Omega)$ and $y_1$ being a regular point of $f$
  is given by
  \begin{equation}
    \label{eq:topoDegreeRegular}
    \deg(f,\Omega,y_1) := \sum_{x\in f^{-1}(y_1)} \sgn J_f(x), 
  \end{equation}
  where $J_f(x):=\det f'(x)$. 
  In particular, $\deg(f,\Omega,y)=0$ if $f^{-1}(y)=\emptyset$.

  Second, the \emph{topological degree} of $(g,\Omega, y)\in M$
  with $g\in {\mathcal C}^2(\Omega)$
  is defined as 
  \begin{equation}
    \label{eq:topoDegreeRegular2}
    \left\{
    \begin{array}{l}
      \deg(g,\Omega,y) := \deg(g,\Omega,y_1), \\
      |y_1-y|<\rho(y,g(\partial \Omega))
      := \min_{z\in g(\partial \Omega)} \|y-z\|_2, 
    \end{array}\right.
  \end{equation}
  where $y_1$ is a regular value of $g$
  and $\deg(g,\Omega,y_1)$ is given by (\ref{eq:topoDegreeRegular}).

  Finally, the \emph{topological degree} of $(f,\Omega, y)\in M$
  is defined as 
  \begin{equation}
    \label{eq:topoDegreeRegularFinal}
    \deg(f,\Omega,y) := \deg(g,\Omega,y), 
  \end{equation}
  where $g\in {\mathcal C}^2(\Omega)\cap {\mathcal C}\left(\overline{\Omega}\right)$
  is any map satisfying $\|g-f\|_{\infty}<\rho(y,f(\partial \Omega))$
  and $\deg(g,\Omega,y)$ is given by (\ref{eq:topoDegreeRegular2}).
\end{definition}

The first definition (\ref{eq:topoDegreeRegular})
clearly comes from Corollary \ref{coro:windingNumberInTermsOfJf}; 
 the second definition (\ref{eq:topoDegreeRegular2})
 is based on Sard's theorem
 that singular values form a set of measure zero; 
 the last definition (\ref{eq:topoDegreeRegularFinal})
 is reminiscent of Rouch\'{e}'s theorem in complex analysis.
Altogether, 
(\ref{eq:topoDegreeRegular}), (\ref{eq:topoDegreeRegular2}),
and (\ref{eq:topoDegreeRegularFinal}) form a sequence of well defined concepts 
that apply to the most general case of $f$ being merely continuous;
see \cite[\S 2]{deimling10:_nonlin_funct_analy}
for more details. 

% The condition of $y$ being a regular value of $f$
%  in Definition \ref{def:topoDegree}
%  can be removed by defining
%  $\deg(f,\Omega,y) := \deg(f,\Omega,y^1)$
%  for $(f,\Omega, y)\in M$
%  with $f\in{\mathcal C}^2(\Omega)$,
%  where $\deg(f,\Omega,y^1)$ is given by Definition
%  \ref{def:topoDegree},
%  $y^1$ any regular value of $f$
%  satisfying $|y^1-y|<\rho(y,f(\partial \Omega))$,
%  and $\rho(y,S)$ the distance from the point $y$ to a set $S$.

% The condition of $f\in{\mathcal C}^2(\Omega)$
%  in the previous paragraph 
%  can be further removed by defining $\deg(f,\Omega,y) := \deg(g,\Omega,y)$
%  for $(f,\Omega, y)\in M$, 
%  where $\deg(g,\Omega,y)$ is given by the previous paragraph
%  and 
%  $g\in {\mathcal C}^2(\Omega)\cap {\mathcal C}\left(\overline{\Omega}\right)$
%  is any map satisfying $\|g-f\|_{\infty}<\rho(y,f(\partial \Omega))$.

\begin{theorem}[Product formula]
  \label{thm:productFormulaOfDegree}
  Suppose $\Omega\subset \mathbb{R}^n$ is open and bounded,
  $f\in {\mathcal C}\left(\overline{\Omega}\right)$,
  $g\in{\mathcal C}(\mathbb{R}^n)$,
  and $y\not\in (g\circ f)(\partial \Omega)$. 
  Then 
  \begin{equation}
    \label{eq:productFormulaOfDegree}
    \deg(g\circ f, \Omega, y)
    = \sum_i \deg(f,\Omega,K_i) \deg(g, K_i, y),
  \end{equation}
  where $K_i$'s are the bounded components
  of $\mathbb{R}^n\setminus f(\partial \Omega)$, 
  $\deg(f,\Omega,K_i)=\deg(f,\Omega,y_i)$
  for any $y_i\in K_i$, and 
  the summation has a finite number of nonzero terms.
\end{theorem}
\begin{proof}
  See \cite[\S 5]{deimling10:_nonlin_funct_analy}.
\end{proof}

Denote by ${\mathcal B}_r(x)$ the open $n$-ball with radius $r$
 and center $x$. 
Analogous to the topological multiplicity
 in (\ref{eq:topoMultiplicityDef}),
 the \emph{index of a continuous map}
 $f\in{\mathcal C}\left(\overline{\mathcal B}_{r_0}(x_0)\right)$
 at $x_0$ is defined as
 \begin{equation}
   \label{eq:indexOfContMapRn}
   j(f,x_0) := \deg(f, {\mathcal B}_r(x_0), f(x_0)),
 \end{equation}
 where $r\in (0,r_0)$ is sufficiently small
 such that $f(x)\ne f(x_0)$
 for all $x\in\overline{\mathcal B}_r(x_0)\setminus \{x_0\}$.
Clearly, $j(f,x_0)$ generalizes
 the topological multiplicity $\nu_f(x_0)$ in (\ref{eq:topoMultiplicityDef}).

\begin{lemma}
  \label{lem:indexOfAnalyticFuncViaProductFormula}
  For an analytic function
  $f: \overline{{\mathcal B}_r(x_0)}\rightarrow \mathbb{C}$
  satisfying $f(x)\ne f(x_0)$
  for any $x\in {\mathcal B}_r(x_0)\setminus\{x_0\}$,
  the index $j(f,x_0)$ in (\ref{eq:indexOfContMapRn})
  reduces to $m_0$,
  the algebraic multiplicity of $f$ at $x_0$.
\end{lemma}
\begin{proof}
  Construct a function $g(z) = x_0 + q z$ where $q\in(0,r)$. 
  Then we have
  \begin{displaymath}
    \begin{array}{rl}
      j(f, x_0) &= \deg(f, {\mathcal B}_q(x_0), 0)
                  = \deg(f\circ g, {\mathcal B}_1(0), 0)
      \\
                   & = w(f(g(\partial {\mathcal B}_1(0))),0 )
                     = w(f(\partial {\mathcal B}_q(0))),0)
                     = m_0,
    \end{array}
  \end{displaymath}
  where the first step follows from (\ref{eq:indexOfContMapRn}), 
  the second from Theorem \ref{thm:productFormulaOfDegree},
  the third from Definition \ref{def:topoDegree}
  and Corollary \ref{coro:windingNumberInTermsOfJf}, 
%  the fourth from  $g(z) = x_0 + q z$,
  and the last from Theorem \ref{thm:argumentPrincipleAnalytic}.
\end{proof}

In the second step of the above proof,
 although $J_f(x_0)=0$ for $m_0>1$, 
 we have $J_{f\circ g}(0) \ne 0$.
Hence the product formula indeed helps in the case of a critical point.

Now we show that the topological degree indeed
 generalizes the winding number.

\begin{theorem}
  \label{thm:TopoDegreeReduceToWindingNumbers}
  For $n=2$,
  the topological degree in Definition \ref{def:topoDegree}
  reduces to the winding number in (\ref{eq:windingNumber}). 
\end{theorem}
\begin{proof}
  At each preimage $z_j$ of $y$,
  either $J_f(z_j)\ne 0$ or $J_f(z_j)= 0$.
  The former case is covered by the same form
  of (\ref{eq:windingNumberViaJacobian}) and
  (\ref{eq:topoDegreeRegular})
  while the latter case
  by Lemma \ref{lem:indexOfAnalyticFuncViaProductFormula}.
\end{proof}

The last major result of this subsection is
 an argument principle in $\mathbb{R}^n$
 via the topological degree,
 which will be useful
 in determining the fluxing index in $\mathbb{R}^n$.

\begin{theorem}
  \label{thm:arguPrincipleViaTopoDegree}
  For the topological degree $d$ in Definition \ref{def:topoDegree},
  we have
  \begin{equation}
    \label{eq:arguPrincipleViaTopoDegree}
    \deg(f,\Omega,y) = \sum_{z_j\in f^{-1}(y)} j(f, z_j),
  \end{equation}
  where $j(f,z_j)$ is given by (\ref{eq:indexOfContMapRn}). 
\end{theorem}
\begin{proof}
  This follows from (TPD-2) in Theorem
  \ref{thm:topoDegreeRnExistence},
  Hopf's theorem in $\mathbb{R}^n$, 
  the definition (\ref{eq:indexOfContMapRn}),
  and the fact that $j(f, z_j)=\pm 1$
  at a preimage $z_j$ satisfying $J_f(z_j)\ne 0$.
\end{proof}


 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../LFC3D"
%%% End:

% LocalWords:  axiomizing preimage BCJ dimensionality nonnegative LFC
% LocalWords:  eversion Jacobian homotopic injective hypersurface
% LocalWords:  homotopy additivity

